EMOTE: An Explainable architecture for Modelling the Other Through Empathy

We can usually assume others have goals analogous to our own. This assumption can also, at times, be applied to multi-agent games - e.g. Agent 1's attraction to green pellets is analogous to Agent 2's attraction to red pellets. This "analogy" assumption is tied closely to the cognitive process known as empathy. Inspired by empathy, we design a simple and explainable architecture to model another agent's action-value function. This involves learning an "Imagination Network" to transform the other agent's observed state in order to produce a human-interpretable "empathetic state" which, when presented to the learning agent, produces behaviours that mimic the other agent. Our approach is applicable to multi-agent scenarios consisting of a single learning agent and other (independent) agents acting according to fixed policies. This architecture is particularly beneficial for (but not limited to) algorithms using a composite value or reward function. We show our method produces better performance in multi-agent games, where it robustly estimates the other's model in different environment configurations. Additionally, we show that the empathetic states are human interpretable, and thus verifiable.

==> Paper_Sections/Exp_Adversarial.tex <==

In the adversarial environment, the harm rate of the sympathy, empathy (all versions) and benchmark models are lower than that of the selfish agent. Though the win rates were not as high as the selfish agent (however close), our approach was able to outperform the Sympathy baseline (where performance decreased over time). For the empathetic run where the button status was manually swapped, performance was better in terms of reducing the harm rate compared to the case of the modeled button. 
%(harming agent As a result of this, the learning agent infers that how the independent agent behaves when the button status is active (when the learning agent has the ability to harm) is much the same as how itself feels when the independent agent can harm. The reverse is true for situations when the button status is inactive.

\iffalse
\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{2a_harmH_Adversarial1}
         \caption{Harm Rate}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{2a_winrate_Adversarial1}
         \caption{Win Rate}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{11a_Adversarial1}
         \caption{$\beta$}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{2a_harmH_Adversarial2}
         \caption{Harm Rate}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{2a_winrate_Adversarial2}
         \caption{Win Rate}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{11a_Adversarial2}
         \caption{$\beta$}
     \end{subfigure}
        \caption{\textbf{Adversarial 1}: (a) - (b) Comparison between Feature and Image-based Empathetic Architecture (manual and modeled button), Sympathetic Agent, Selfish agent and two benchmarks. (c) win rate and door open rate as $\delta$ is varied, averaged over the last 100 episodes.}
        \label{fig:Adversarial1 Results}
\end{figure*}
\fi


\iffalse
\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{11a_GridworldAss1}
         \caption{Assistive 1}
     \end{subfigure}
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{11a_GridworldAss2}
         \caption{Assistive 2}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{11a_Adversarial1}
         \caption{Adversarial 1}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{11a_Adversarial2}
         \caption{Adversarial 2}
     \end{subfigure}
        \caption{\textbf{Adversarial}: (a) - (b) Comparison between Feature and Image-based Empathetic Architecture (manual and modeled button), Sympathetic Agent, Selfish agent and two benchmarks. (c) win rate and door open rate as $\delta$ is varied, averaged over the last 100 episodes.}
        \label{fig:beta_results}
\end{figure*}
\fi

==> Paper_Sections/Exp_Assistive.tex <==
\iffalse
\begin{figure*}[ht]
     \centering
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{2a_door_GridworldAss1}
         \caption{Assistive 1: Door open rate}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{2a_winrate_GridworldAss1}
         \caption{Assistive 1: Win Rate}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{11a_GridworldAss1}
         \caption{Assistive 1: Varying $\delta$}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{2a_door_GridworldAss2}
         \caption{Assistive 2: Door open rate}
     \end{subfigure}
     \begin{subfigure}[b]{0.30\textwidth}
         \centering
         \includegraphics[width=\textwidth]{2a_winrate_GridworldAss2}
         \caption{Assistive 2: Win Rate}
     \end{subfigure}
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{11a_GridworldAss2}
         \caption{Assistive 2: Varying $\delta$}
     \end{subfigure}
        \caption{Comparison between Feature and Image-based Empathetic Architecture, Sympathetic Agent, Selfish agent and two benchmarks. (c) and (f) Empathetic IRL reward values, averaged over the last 100 episodes.}
        \label{fig:Assistive Results}
\end{figure*}
\fi

\begin{table*}[]
\begin{center}
\begin{tabular}{|c|ll|ll|ll|ll|}
\hline
{\color[HTML]{000000} } & \multicolumn{2}{c|}{{\color[HTML]{000000} Assistive 1}} & \multicolumn{2}{c|}{{\color[HTML]{000000} Assistive 2}} & \multicolumn{2}{c|}{{\color[HTML]{000000} Adversarial 1}} & \multicolumn{2}{c|}{{\color[HTML]{000000} Adversarial 2}} \\ \hline
{\color[HTML]{000000} } & \multicolumn{1}{c|}{{\color[HTML]{000000} Door}} & \multicolumn{1}{c|}{{\color[HTML]{000000} Win}} & \multicolumn{1}{c|}{{\color[HTML]{000000} Door}} & \multicolumn{1}{c|}{{\color[HTML]{000000} Win}} & \multicolumn{1}{c|}{{\color[HTML]{000000} Harm}} & \multicolumn{1}{c|}{{\color[HTML]{000000} Win}} & \multicolumn{1}{c|}{{\color[HTML]{000000} Harm}} & \multicolumn{1}{c|}{{\color[HTML]{000000} Win}} \\ \hline
{\color[HTML]{000000} Selfish} & \multicolumn{1}{l|}{{\color[HTML]{000000} 0.44$\pm$0.15}} & {\color[HTML]{000000} 0.8$\pm$0.11} & \multicolumn{1}{l|}{{\color[HTML]{000000} 0.09$\pm$0.07}} & {\color[HTML]{000000} 0.89$\pm$0.08} & \multicolumn{1}{l|}{{\color[HTML]{000000} 0.5$\pm$0.15}} & {\color[HTML]{000000} 0.46$\pm$0.15} & \multicolumn{1}{l|}{{\color[HTML]{000000} 0.29$\pm$0.13}} & {\color[HTML]{000000} 0.73$\pm$0.13} \\ \hline
{\color[HTML]{000000} Sympathy} & \multicolumn{1}{l|}{{\color[HTML]{000000} \textbf{0.99$\pm$0.01}}} & {\color[HTML]{000000} \textbf{0.93$\pm$0.05}} & \multicolumn{1}{l|}{{\color[HTML]{000000} \textbf{0.17$\pm$0.1}}} & {\color[HTML]{000000} \textbf{0.92$\pm$0.06}} & \multicolumn{1}{l|}{{\color[HTML]{000000} \textbf{0.45$\pm$0.15}}} & {\color[HTML]{000000} 0.26$\pm$0.13} & \multicolumn{1}{l|}{{\color[HTML]{000000} \textbf{0.12$\pm$0.09}}} & {\color[HTML]{000000} 0.31$\pm$0.14} \\ \hline
{\color[HTML]{000000} E-Feature} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.99$\pm$0.01}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.93$\pm$0.05}} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.4$\pm$0.15}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.94$\pm$0.05}} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.24$\pm$0.12}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} 0.4$\pm$0.15} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.1$\pm$0.08}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} 0.44$\pm$0.15} \\ \hline
{\color[HTML]{000000} E-Image} & \multicolumn{1}{l|}{{\color[HTML]{000000} \textbf{0.83$\pm$0.11}}} & {\color[HTML]{000000} \textbf{0.92$\pm$0.06}} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.38$\pm$0.15}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.92$\pm$0.06}} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.17$\pm$0.1}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} 0.41$\pm$0.15} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.12$\pm$0.09}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} 0.47$\pm$0.15} \\ \hline
{\color[HTML]{000000} B-Vis} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{1$\pm$0}}} & {\color[HTML]{000000} \textbf{0.92$\pm$0.06}} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.21$\pm$0.11}}} & {\color[HTML]{000000} \textbf{0.89$\pm$0.08}} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.1$\pm$0.07}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} 0.37$\pm$0.15} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.05$\pm$0.04}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} 0.34$\pm$0.14} \\ \hline
{\color[HTML]{000000} B-Invis} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{1$\pm$0}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.93$\pm$0.05}} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.19$\pm$0.11}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.92$\pm$0.06}} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.1$\pm$0.07}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} 0.34$\pm$0.14} & \multicolumn{1}{l|}{\cellcolor[HTML]{9AC68B}{\color[HTML]{000000} \textbf{0.03$\pm$0.02}}} & \cellcolor[HTML]{9AC68B}{\color[HTML]{000000} 0.33$\pm$0.14} \\ \hline
\end{tabular}
\caption{Performance results of all environments. Assistive games show rate of win and door being opened. Adversarial games show rate of win and harm from the learning agent towards the independent agent. Cells highlighted in green are those in which the performance was better than the Sympathy run. Cells with bold text are those, compared with the Selfish run, in which intended considerate behaviour was achieved and comparable win rates were also achieved.}
\label{table:win_harm_door}
\end{center}
\end{table*}
\vspace*{-\baselineskip}

Table \ref{table:win_harm_door} shows the Win Rate and Door Open rate for the two Assistive environments, as well as the Win Rate and Harm Rate (rate at which the learning agent harms the independent agent) for each of the adversarial runs. In the Assistive environments the Feature and Image-based Empathy models result in high win and door open rates. A door open rate close to 1 indicates that the door was opened consistently in each run, while a value close to 0 indicates the door was not opened often. In fact, the performance was even higher than the benchmarks and Sympathy baseline for opening the door. The Feature-based Empathy model opens the door at a similar or better rate than Sympathy.

\iffalse
\begin{table*}[]
\caption{Average inferred rewards for Assistive games. First row is learning agent's rewards returned from the environment. All subsequent rows are inferred rewards for the independent agent from $\hat{Q}_{indep}$ via IRL}
\begin{center}
\begin{tabular}{lllllllllll}
\hline
\multicolumn{1}{|l|}{}             & \multicolumn{5}{c|}{Assistive 1}                                                                                                              & \multicolumn{5}{c|}{Assistive 2}                                                                                                              \\ \hline
\multicolumn{1}{|l|}{}             & \multicolumn{1}{l|}{IP}   & \multicolumn{1}{l|}{LP}    & \multicolumn{1}{l|}{D}     & \multicolumn{1}{l|}{W}     & \multicolumn{1}{l|}{S}     & \multicolumn{1}{l|}{IP}   & \multicolumn{1}{l|}{LP}    & \multicolumn{1}{l|}{D}     & \multicolumn{1}{l|}{W}     & \multicolumn{1}{l|}{S}     \\ \hline
\rowcolor[HTML]{C0C0C0} 
Env. Rewards                       & 0                         & 10                         & -1                         & 5                          & -1                         & 0                         & 10                         & -1                         & 5                          & -1                         \\ \hline
\multicolumn{1}{|l|}{Emp(Feature)} & \multicolumn{1}{l|}{2.95} & \multicolumn{1}{l|}{-1.31} & \multicolumn{1}{l|}{3.49}  & \multicolumn{1}{l|}{0.1}   & \multicolumn{1}{l|}{-1.52} & \multicolumn{1}{l|}{3.38} & \multicolumn{1}{l|}{-1.04} & \multicolumn{1}{l|}{0.94}  & \multicolumn{1}{l|}{0.51}  & \multicolumn{1}{l|}{-1.19} \\ \hline
\multicolumn{1}{|l|}{Emp(Image)}   & \multicolumn{1}{l|}{0.34} & \multicolumn{1}{l|}{-0.64} & \multicolumn{1}{l|}{0.17}  & \multicolumn{1}{l|}{-0.21} & \multicolumn{1}{l|}{-1.07} & \multicolumn{1}{l|}{0.51} & \multicolumn{1}{l|}{-0.62} & \multicolumn{1}{l|}{1.48}  & \multicolumn{1}{l|}{0}     & \multicolumn{1}{l|}{-0.92} \\ \hline
\multicolumn{1}{|l|}{Sympathy}     & \multicolumn{1}{l|}{1.09} & \multicolumn{1}{l|}{-0.69} & \multicolumn{1}{l|}{13.87} & \multicolumn{1}{l|}{-0.13} & \multicolumn{1}{l|}{-0.93} & \multicolumn{1}{l|}{3.19} & \multicolumn{1}{l|}{-1.54} & \multicolumn{1}{l|}{-5.65} & \multicolumn{1}{l|}{-0.05} & \multicolumn{1}{l|}{-1.96} \\ \hline
\multicolumn{1}{|l|}{B-Visible}    & \multicolumn{1}{l|}{7.28} & \multicolumn{1}{l|}{-1.78} & \multicolumn{1}{l|}{-9.03} & \multicolumn{1}{l|}{0.58}  & \multicolumn{1}{l|}{-1.91} & \multicolumn{1}{l|}{6.67} & \multicolumn{1}{l|}{-1.55} & \multicolumn{1}{l|}{-1.61} & \multicolumn{1}{l|}{1.2}   & \multicolumn{1}{l|}{-2.2}  \\ \hline
\multicolumn{1}{|l|}{B-Invisible}  & \multicolumn{1}{l|}{6.17} & \multicolumn{1}{l|}{-1.73} & \multicolumn{1}{l|}{-5.95} & \multicolumn{1}{l|}{1}     & \multicolumn{1}{l|}{-1.94} & \multicolumn{1}{l|}{6.86} & \multicolumn{1}{l|}{-1.55} & \multicolumn{1}{l|}{-2.43} & \multicolumn{1}{l|}{1.1}   & \multicolumn{1}{l|}{-2.14} \\ \hline
\multicolumn{1}{|l|}{B-Recolor}    & \multicolumn{1}{l|}{7.68} & \multicolumn{1}{l|}{-2.13} & \multicolumn{1}{l|}{-2.26} & \multicolumn{1}{l|}{1.16}  & \multicolumn{1}{l|}{-2.38} & \multicolumn{1}{l|}{6.66} & \multicolumn{1}{l|}{-1.56} & \multicolumn{1}{l|}{-0.41} & \multicolumn{1}{l|}{1.39}  & \multicolumn{1}{l|}{-2.07} \\ \hline
\end{tabular}
\label{table:Assistive_rewards}
\end{center}
\end{table*}
\fi





==> Paper_Sections/adapt_cascaded.tex <==
\thommen{Is this subsection needed? Can it be fit into the text surrounding Eq 2? Many points here are repeated there anyway.}In the Sympathy Framework paper, the authors utilised the Cascaded Supervised Learning method \cite{cascadedSuperIRL2013} to conduct the IRL to infer the value function and rewards for the independent agent. The method involves two stages. In the first, a supervised learning approach is applied using observed state-action pairs of the independent agent to train a value function. In the second stage, this value function is used within a rearranged form of the Bellman equation \cite{sutton2018reinforcement} to extract a form of the inferred reward function for the independent agent. This method has been shown to be a successful means of extracting a reward function that produces a policy that mimics the independent agent's behaviour. However, the method still suffers a key issue faced by most IRL methods - that there exists a vast space of potential reward functions that when rolled out, could express the observed behaviour of an agent \cite{PolicyInvariance}. 
Under the assumption that both agents are similar (in terms of goals and underlying reward values) our proposed method is to change the value function of the method to our empathy-based architecture. In this way, the resulting value function and rewards will be more comparable and consistent between both agents thereby addressing some of the shortcomings of the Sympathy Framework method, as was discussed in the Related Literature section.  

%In the Sympathy Framework paper, in order to constrain the space of rewards to those which are appropriate for comparing against the rewards of the learning agent (an important consideration when producing the sympathetic rewards to train the learning agent), the authors scale the inferred rewards of the independent agent to have the same $L_{1}$ norm as that of the learning agent's reward function. This however still does not guarantee that the reward inferred is in fact appropriately comparable to that of the learning agent. In addition, it requires that the the learning agent's reward function be known before hand fully, which may not always be the case (such as cases where the reward values only exposed to the agent as it interacts with the environment).\thommen{Again, its okay to contrast the work with the sympathy paper, but maybe it should be reserved for the related works/discussion sections. I feel like the focus is being lost.}


==> Paper_Sections/algorithm.tex <==
Algorithm \ref{alg:IRL_1} presents the pseudocode for updating the empathy-based value function of the independent agent. 

\begin{algorithm}[h]
    \caption{Independent Agent Value Function Update}
	\label{alg:IRL_1}
	\begin{flushleft}
    \textbf{Inputs}: Indep. Agent Replay Memory $D_{indep}$, $\hat{Q}_{indep}$\\
	\end{flushleft}
	\begin{algorithmic}[1] %[1] enables line numbers
	    \STATE Sample random batch of transitions from $D_{indep}$
		\FOR{$j = 1, 2, ..., batch$}
		\STATE $s_{e_{j}} = M_{imagine}(s_{j} ; \theta_{imagine})$
		\STATE Set $y_{j}$ = $\mathbbm{1}.a_{j}^{indep}$\text{(one-hot encoded actions)}
		\STATE Update $\theta_{imagine}$ w.r.t loss (Eqn \ref{eqn:Loss_Function})
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

\iffalse
\STATE $\pi(a_{j}|s_{j})=\frac{e^{\hat{Q_{indep}(s_{j},a_{j};\theta_{indep})}}}{\sum_{a}e^{\hat{Q_{indep}(s_{j},a;\theta_{indep})}}}$ 
\STATE
$\theta_{indep} = [\theta_{imagine},\theta_{selfish}]$
\STATE $\frac{1}{n}\sum\left((1-\delta)\text{CE}(y_{j},\pi(a_{j}|s_{j})) + \delta\norm{s_{j} - s^{i}_{j}}\right)$
\fi


==> Paper_Sections/performance_table.tex <==
\begin{table*}
\vskip -0.3in
\begin{center}
\caption{Performance results. Assistive games show win rate (higher is better) and door-opening rate (higher is better). Adversarial games show win rate (higher is better) and harm rate (lower is better) from the learning agent toward the independent agent. Cells are shaded green where performance exceeded Sympathy. Cells have bold text where intended considerate behaviour or comparable win rates were achieved, compared to Selfish run.}
\vskip 0.15in
\begin{tabular}{lcccccccl}
\toprule
& & \multicolumn{1}{c}{Selfish} & \multicolumn{1}{c}{Sympathy} & \multicolumn{1}{c}{E-Feature} & \multicolumn{1}{c}{E-Image} & \multicolumn{1}{c}{B-Vis} & \multicolumn{1}{c}{B-Invis} \\ \midrule 
 & Door & 0.44$\pm$0.15 & \textbf{0.99$\pm$0.01} & \cellcolor[HTML]{9AC68B}\textbf{0.99$\pm$0.01} & \textbf{0.83$\pm$0.11} & \cellcolor[HTML]{9AC68B}\textbf{1$\pm$0} & \cellcolor[HTML]{9AC68B}\textbf{1$\pm$0} \\ \cline{8-8} 
\multirow{Ass. 1} & Win & 0.8$\pm$0.11 & \textbf{0.93$\pm$0.05} & \cellcolor[HTML]{9AC68B}\textbf{0.93$\pm$0.05} & \textbf{0.92$\pm$0.06} & \textbf{0.92$\pm$0.06} & \cellcolor[HTML]{9AC68B}\textbf{0.93$\pm$0.05} \\ \midrule 
 & Door & 0.09$\pm$0.07 & \textbf{0.17$\pm$0.1} & \cellcolor[HTML]{9AC68B}\textbf{0.4$\pm$0.15} & \cellcolor[HTML]{9AC68B}\textbf{0.38$\pm$0.15} & \cellcolor[HTML]{9AC68B}\textbf{0.21$\pm$0.11} & \cellcolor[HTML]{9AC68B}\textbf{0.19$\pm$0.11} \\ \cline{8-8} 
\multirow{Ass. 2} & Win & 0.89$\pm$0.08 & \textbf{0.92$\pm$0.06} & \cellcolor[HTML]{9AC68B}\textbf{0.94$\pm$0.05} & \cellcolor[HTML]{9AC68B}\textbf{0.92$\pm$0.06} & \textbf{0.89$\pm$0.08} & \cellcolor[HTML]{9AC68B}\textbf{0.92$\pm$0.06} \\ \midrule  
 & Harm & 0.5$\pm$0.15 & \textbf{0.45$\pm$0.15} & \cellcolor[HTML]{9AC68B}\textbf{0.24$\pm$0.12} & \cellcolor[HTML]{9AC68B}\textbf{0.17$\pm$0.1} & \cellcolor[HTML]{9AC68B}\textbf{0.1$\pm$0.07} & \cellcolor[HTML]{9AC68B}\textbf{0.1$\pm$0.07} \\ \cline{8-8} 
\multirow{Adv. 1} & Win & 0.46$\pm$0.15 & 0.26$\pm$0.13 & \cellcolor[HTML]{9AC68B}0.4$\pm$0.15 & \cellcolor[HTML]{9AC68B}0.41$\pm$0.15 & \cellcolor[HTML]{9AC68B}0.37$\pm$0.15 & \cellcolor[HTML]{9AC68B}0.34$\pm$0.14 \\ \midrule
 & Harm & 0.29$\pm$0.13 & \textbf{0.12$\pm$0.09} & \cellcolor[HTML]{9AC68B}\textbf{0.1$\pm$0.08} & \cellcolor[HTML]{9AC68B}\textbf{0.12$\pm$0.09} & \cellcolor[HTML]{9AC68B}\textbf{0.05$\pm$0.04} & \cellcolor[HTML]{9AC68B}\textbf{0.03$\pm$0.02} \\ \cline{8-8} 
\multirow{Adv. 2} & Win & 0.73$\pm$0.13 & 0.31$\pm$0.14 & \cellcolor[HTML]{9AC68B}0.44$\pm$0.15 & \cellcolor[HTML]{9AC68B}0.47$\pm$0.15 & \cellcolor[HTML]{9AC68B}0.34$\pm$0.14 & \cellcolor[HTML]{9AC68B}0.33$\pm$0.14 \\\midrule
\end{tabular}
\label{table:win_harm_door}
\end{center}
\vskip -0.3in
\end{table*}
